Unified Parameter-Efficient Unlearning for LLMs

The advent of Large Language Models (LLMs) has revolutionized natural language processing, enabling advanced understanding and reasoning capabilities across a variety of tasks. Fine-tuning these models for specific domains, particularly through Parameter-Efficient Fine-Tuning (PEFT) strategies like LoRA, has become a prevalent practice due to its efficiency. However, this raises significant privacy and security concerns, as models may inadvertently retain and disseminate sensitive or undesirable information. To address these issues, we introduce a novel instance-wise unlearning framework, LLMEraser, which systematically categorizes unlearning tasks and applies precise parameter adjustments using influence functions. Unlike traditional unlearning techniques that are often limited in scope and require extensive retraining, LLMEraser is designed to handle a broad spectrum of unlearning tasks without compromising model performance. Extensive experiments on benchmark datasets demonstrate that LLMEraser excels in efficiently managing various unlearning scenarios while maintaining the overall integrity and efficacy of the models.

==> chapters/6_related_work.tex <==
\section{Related Work}
\subsection{Large Language Models}
Recent advancements in natural language processing (NLP) \citep{DBLP:conf/icse/NamMHVM24,DBLP:journals/corr/abs-2401-01325} have been significantly driven by the development of pretrained language models and Large Language Models. The introduction of models like BERT \citep{DBLP:conf/naacl/DevlinCLT19} and GPT-2 \citep{radford2019language} marked a pivotal shift in leveraging large-scale unsupervised pretraining, enabling superior performance across various NLP tasks through fine-tuning. The scaling of language models led to the emergence of LLMs such as GPT-3 \citep{DBLP:conf/nips/BrownMRSKDNSSAA20} and PaLM \citep{DBLP:journals/jmlr/ChowdheryNDBMRBCSGSSTMRBTSPRDHPBAI23}, which have pushed the boundaries of language understanding and generation. These models, with billions of parameters, are capable of performing complex reasoning and handling diverse tasks with minimal instruction.

Recent research has explored parameter-efficient fine-tuning techniques, which adapt large models to specific applications without requiring extensive computational resources. Techniques like Adapter modules \citep{DBLP:conf/icml/HoulsbyGJMLGAG19} and Low-Rank Adaptation (LoRA) \citep{DBLP:conf/iclr/HuSWALWWC22} have gained popularity for their efficiency and effectiveness in maintaining performance while reducing the number of trainable parameters. Furthermore, instruction tuning \citep{DBLP:journals/corr/abs-2310-03744,DBLP:conf/sigir/Tang00SSCY024} using domain-specific data has emerged as a key strategy to enhance model performance in specialized contexts. Works by \cite{DBLP:conf/nips/Ouyang0JAWMZASR22} and \cite{dodge2020fine} illustrate how tailoring models to specific tasks through targeted instruction can significantly improve their utility, particularly in complex domains, demonstrating the importance of context and relevance in model training.

LLMs have found extensive applications in various downstream tasks, demonstrating their versatility across domains such as natural language processing, information retrieval, and knowledge graph augmentation \citep{DBLP:journals/corr/abs-2401-11181,DBLP:conf/iclr/0006LCF24,DBLP:journals/imwut/XuYDGYHGDW24}. For instance, LLMs are employed to enhance the accuracy of query-based systems by leveraging their ability to understand and generate contextually relevant responses, improving user experience in search applications \citep{DBLP:journals/corr/abs-2401-02038,DBLP:journals/corr/abs-2404-14809}. Additionally, they are utilized in graph analytics, enabling complex reasoning tasks and facilitating the extraction of insights from structured data \citep{DBLP:journals/sigkdd/ChenMLJWWWYFLT23,DBLP:journals/corr/abs-2406-01032}. The adaptability of LLMs through prompt engineering further supports their deployment in specific use cases, allowing for tailored outputs that meet diverse requirements \citep{DBLP:conf/chi/ArawjoSVWG24,cain2024prompting}.

\subsection{Large Language Models Unlearning}
The concept of unlearning in Large Language Models has garnered considerable attention as concerns over data privacy and model integrity have intensified. In-context unlearning, proposed by \cite{pawelczyk2023context}, allows the selective removal of data points by supplying flipped labels during inference, effectively maintaining performance while unlearning specific information. Additionally, Quark by \cite{DBLP:conf/nips/LuWHJQWA022} employs a reinforcement learning framework to control and reduce undesirable behaviors, enhancing text generation without extensive retraining.

\cite{DBLP:conf/emnlp/ChenY23} introduce a lightweight unlearning method that integrates unlearning layers into transformer architectures, facilitating efficient data removal. Knowledge Unlearning by \cite{DBLP:conf/acl/JangYYCLLS23} demonstrates that targeted gradient ascent can effectively forget sensitive information, surpassing traditional methods in performance retention. The technique proposed by \cite{DBLP:journals/corr/abs-2310-02238} facilitates the removal of specific facts related to the Harry Potter series while preserving the model's overall performance.

Other approaches, such as the Partitioned Gradient Update (PGU) method by \cite{DBLP:conf/acl/YuJKYJ23}, aim to reduce social biases effectively. Collectively, these studies underline the significance of unlearning in LLMs, paving the way for safer, more responsible AI applications.



==> chapters/7_limitation.tex <==
\section{Limitations}
LLMEraser offers efficient parameter updates without the need for retraining, making it versatile across different unlearning tasks while also reducing computational overhead. 
Despite the improvements brought by LLMEraser, its potential shortcomings should not be overlooked. Calculating parameter changes for different unlearning tasks requires accessing the gradient information of the target data and assumes availability of the training set. Furthermore, the influence function's reliance on the first-order Taylor expansion of the optimization objective leads to the inevitable estimation errors, representing an inherent limitation of such approach.
